Modified BART for Learning Heterogeneous Effects in Regression Discontinuity Designs

This paper introduces BART-RDD, a sum-of-trees regression model built around a novel regression tree prior, which incorporates the special covariate structure of regression discontinuity designs. Specifically, the tree splitting process is constrained to ensure overlap within a narrow band surrounding the running variable cutoff value, where the treatment effect is identified. It is shown that unmodified BART-based models estimate RDD treatment effects poorly, while our modified model accurately recovers treatment effects at the cutoff. Specifically, BART-RDD is perhaps the first RDD method that effectively learns conditional average treatment effects. The new method is investigated in thorough simulation studies as well as an empirical application looking at the effect of academic probation on student performance in subsequent terms (Lindo et al., 2010).

==> Figures/cart_gpa.tex <==
\begin{figure}[!htpb]
	\centering
	\includegraphics[scale=0.5]{Figures/gpa_cart_2.pdf}
	\caption{CART tree for individual treatment effects}
	\label{fig:cart.gpa}
\end{figure}

==> Figures/cate.tex <==
\begin{figure}[!htpb]
	\centering
	\begin{subfigure}[b]{0.45\textwidth}
		\centering
		\includegraphics[width=\textwidth]{Figures/post_age.png}
		\caption{CATE posterior by age}
		\label{fig:cate.a}
	\end{subfigure}
	\hfill
	\begin{subfigure}[b]{0.45\textwidth}
		\centering
		\includegraphics[width=\textwidth]{Figures/post_grade.png}
		\caption{CATE posterior by high school grade percentile}
		\label{fig:cate.b}
	\end{subfigure}
	\hfill
	\begin{subfigure}[b]{0.45\textwidth}
		\centering
		\includegraphics[width=\textwidth]{Figures/post_diff_camp_1.png}
		\caption{$\Delta_1$}
		\label{fig:cate.c}
	\end{subfigure}
	\hfill
	\begin{subfigure}[b]{0.45\textwidth}
		\centering
		\includegraphics[width=\textwidth]{Figures/post_diff_camp_2.png}
		\caption{$\Delta_2$}
		\label{fig:cate.d}
	\end{subfigure}
	\caption{Heterogeneity in $\tau$ posterior}
	\label{fig:cate}
\end{figure}

==> Figures/cate_results.tex <==
\begin{figure}
	\centering
	\begin{subfigure}[b]{0.45\textwidth}
		\centering
		\includegraphics[width=\textwidth]{Figures/rmse_cate.png}
		\caption{RMSE}
		\label{fig:rmse.cate}
	\end{subfigure}
	\hfill
	\begin{subfigure}[b]{0.45\textwidth}
		\centering
		\includegraphics[width=\textwidth]{Figures/coverage_cate.png}
		\caption{Coverage x Length}
		\label{fig:coverage.cate}
	\end{subfigure}
	\caption{CATE results}
	\label{fig:cate_results}
\end{figure}

==> Figures/corrected_coverage.tex <==
\begin{figure}
	\centering
	\begin{subfigure}[b]{0.45\textwidth}
		\centering
		\includegraphics[width=\textwidth]{Figures/length1.png}
		\caption{Model 1 and 2}
		\label{fig:length.a}
	\end{subfigure}
	\hfill
	\begin{subfigure}[b]{0.45\textwidth}
		\centering
		\includegraphics[width=\textwidth]{Figures/length2.png}
		\caption{Model 3 and 4}
		\label{fig:length.b}
	\end{subfigure}
	\caption{Corrected 95\% Interval Length}
	\label{fig:length_ate}
\end{figure}

==> Figures/coverage_ate.tex <==
\begin{figure}
	\centering
	\begin{subfigure}[b]{0.45\textwidth}
		\centering
		\includegraphics[width=\textwidth]{Figures/coverage1.png}
		\caption{Model 1 and 2}
		\label{fig:coverage.a}
	\end{subfigure}
	\hfill
	\begin{subfigure}[b]{0.45\textwidth}
		\centering
		\includegraphics[width=\textwidth]{Figures/coverage2.png}
		\caption{Model 3 and 4}
		\label{fig:coverage.b}
	\end{subfigure}
	\caption{Coverage x Length}
	\label{fig:coverage_ate}
\end{figure}

==> Figures/coverage_cate.tex <==
\begin{figure}
	\centering
	\includegraphics[scale=0.6]{Figures/coverage_cate.png}
	\caption{Coverage x Length}
	\label{fig:coverage.cate}
\end{figure}

==> Figures/gpa.tex <==
\begin{figure}
	\centering
	\begin{subfigure}[b]{0.45\textwidth}
		\centering
		\includegraphics[width=\textwidth]{Figures/gpa_data.png}
		\caption{Scatter plot}
		\label{fig:gpa.a}
	\end{subfigure}
	\hfill
	\begin{subfigure}[b]{0.45\textwidth}
		\centering         \includegraphics[width=\textwidth]{Figures/gpa.png}
		\caption{Loess Fit}
		\label{fig:gpa.b}
	\end{subfigure}
	\caption{Second x First Year GPA}
	\label{fig:gpa}
\end{figure}

==> Figures/gpa_dist.tex <==
\begin{figure}
	\centering
	\includegraphics[scale=0.7]{Figures/gpa_cutoff_dist.png}
	\caption{First Year GPA Distribution}
	\label{fig:gpa.dist}
\end{figure}

==> Figures/grades.tex <==
\begin{figure}
	\centering
	\begin{subfigure}[b]{0.45\textwidth}
		\centering
		\includegraphics[width=\textwidth]{Figures/grades_dist.png}
		\caption{Density}
		\label{fig:grades.a}
	\end{subfigure}
	\hfill
	\begin{subfigure}[b]{0.45\textwidth}
		\centering         \includegraphics[width=\textwidth]{Figures/grades_score.png}
		\caption{Scatter plot}
		\label{fig:grades.b}
	\end{subfigure}
	\caption{High school grade percentile}
	\label{fig:grades}
\end{figure}

==> Figures/prior.tex <==
\begin{figure}[!htpb]
	\centering
	\begin{subfigure}[b]{0.45\textwidth}
		\centering
		\includegraphics[width=\textwidth]{Figures/prior_true_1.pdf}
		\caption{$E(Y)$}
		\label{fig:prior.a}
	\end{subfigure}
	\hfill
	\begin{subfigure}[b]{0.45\textwidth}
		\centering
		\includegraphics[width=\textwidth]{Figures/prior_true_2.pdf}
		\caption{$Y$}
		\label{fig:prior.b}
              \end{subfigure}
              \caption{True data}
              \label{fig:prior.1}
\end{figure}

==> Figures/prior_model.tex <==
\begin{figure}[!htpb]
	\centering
	\includegraphics[width=0.75\linewidth]{Figures/prior_true_1.pdf}
	\caption{Prognostic, treatment effect and mean functions for the true DGP considered in the illustration of the prior elicitation procedure}
	\label{fig:prior.1}
\end{figure}

==> Figures/prior_sensitivity.tex <==
\begin{figure}[!htpb]
	\centering
	\begin{subfigure}[b]{0.49\textwidth}
		\centering
		\includegraphics[width=\textwidth]{Figures/prior_omin1.pdf}
		\caption{$X_1$}
		\label{fig:prior.omin.a}
	\end{subfigure}
	\hfill
	\begin{subfigure}[b]{0.49\textwidth}
		\centering
		\includegraphics[width=\textwidth]{Figures/prior_omin2.pdf}
		\caption{$X_2$}
		\label{fig:prior.omin.b}
	\end{subfigure}
	\hfill
	\begin{subfigure}[b]{0.49\textwidth}
		\centering
		\includegraphics[width=\textwidth]{Figures/prior_omin3.pdf}
		\caption{$X_3$}
		\label{fig:prior.omin.c}
	\end{subfigure}
	\caption{ATE point estimates for different $N_{Omin}$
		and $\alpha$}
	\label{fig:prior.omin}
\end{figure}

==> Figures/prior_sensitivity_1.tex <==
\begin{figure}[!htpb]
	\centering
	\begin{subfigure}[b]{0.49\linewidth}
		\centering
		\includegraphics[width=\linewidth]{Figures/prior_omin1.pdf}
		\caption{$X_1$}
		\label{fig:prior.omin.a}
	\end{subfigure}
	\hfill
	\begin{subfigure}[b]{0.49\linewidth}
		\centering
		\includegraphics[width=\linewidth]{Figures/prior_omin2.pdf}
		\caption{$X_2$}
		\label{fig:prior.omin.b}
	\end{subfigure}
	\hfill
	\begin{subfigure}[b]{0.49\linewidth}
		\centering
		\includegraphics[width=\linewidth]{Figures/prior_omin3.pdf}
		\caption{$X_3$}
		\label{fig:prior.omin.c}
	\end{subfigure}
	\caption{ATE point estimates for different $N_{Omin}$
		and $\alpha$ under the selected $h$ value for each variation of the true DGP}
	\label{fig:prior.omin}
\end{figure}

==> Figures/prior_sensitivity_2.tex <==
\begin{figure}[!htpb]
	\centering
	\begin{subfigure}[b]{0.49\linewidth}
		\centering
		\includegraphics[width=\linewidth]{Figures/prior_het_omin1.pdf}
		\caption{$X_1$}
		\label{fig:prior.het.omin.a}
	\end{subfigure}
	\hfill
	\begin{subfigure}[b]{0.49\linewidth}
		\centering
		\includegraphics[width=\linewidth]{Figures/prior_het_omin2.pdf}
		\caption{$X_2$}
		\label{fig:prior.het.omin.b}
	\end{subfigure}
	\hfill
	\begin{subfigure}[b]{0.49\linewidth}
		\centering
		\includegraphics[width=\linewidth]{Figures/prior_het_omin3.pdf}
		\caption{$X_3$}
		\label{fig:prior.het.omin.c}
	\end{subfigure}
	\caption{Groups detected in BART-RDD posterior for
		different $N_{Omin}$ and $\alpha$ under the selected $h$ value for each variation of the true DGP}
	\label{fig:prior.het.omin}
\end{figure}

==> Figures/rmse_ate.tex <==
\begin{figure}
	\centering
	\begin{subfigure}[b]{0.45\textwidth}
		\centering
		\includegraphics[width=\textwidth]{Figures/rmse1.png}
		\caption{Model 1 and 2}
		\label{fig:rmse.a}
	\end{subfigure}
	\hfill
	\begin{subfigure}[b]{0.45\textwidth}
		\centering
		\includegraphics[width=\textwidth]{Figures/rmse2.png}
		\caption{Model 3 and 4}
		\label{fig:rmse.b}
	\end{subfigure}
	\caption{RMSE}
	\label{fig:rmse_ate}
\end{figure}

==> Figures/rmse_cate.tex <==
\begin{figure}
	\centering
	\includegraphics[scale=0.6]{Figures/rmse_cate.png}
	\caption{RMSE}
	\label{fig:rmse.cate}
\end{figure}

==> Figures/sim_coverage_ate.tex <==
\begin{figure}[!htpb]
	\centering
	\includegraphics[width=0.75\linewidth]{Figures/sim_intervals.pdf}
	\caption{Confidence intervals for the ATE produced by each estimator, divided by different levels of heterogenety (\textit{i.e.} $\kappa$)}
	\label{fig:sim.int.ate}
\end{figure}

==> Figures/sim_data.tex <==
\begin{figure}
	\centering
	\includegraphics[width=0.75\linewidth]{Figures/sim_dgp_1.pdf}
	\caption{Prognostic and treatment effect functions by
		heterogeneity level: the first row represents the
		prognostic functions, the second represents the
		treatment effect functions; each column represents,
		respectively, $\kappa = \{0,1,2\}$}
	\label{fig:sim.dgp}
\end{figure}

==> Figures/sim_functions.tex <==
\begin{figure}[!htpb]
	\centering
	\includegraphics[width=\textwidth]{Figures/sim_mu_tau.pdf}
	\caption{Prognostic and treatment effect functions}
	\label{fig:sim.functions}
\end{figure}

==> Figures/sim_rmse_ate.tex <==
\begin{figure}
	\centering
	\begin{subfigure}[b]{0.49\textwidth}
		\centering
		\includegraphics[width=\textwidth]{Figures/absolute_bias_delta_mu.pdf}
		\caption{$\delta_{\mu}$}
		\label{fig:bias.delta.mu}
	\end{subfigure}
	\hfill
	\begin{subfigure}[b]{0.49\textwidth}
		\centering
		\includegraphics[width=\textwidth]{Figures/absolute_bias_delta_tau.pdf}
		\caption{$\delta_{\tau}$}
		\label{fig:bias.delta.tau}
	\end{subfigure}
	\hfill
	\begin{subfigure}[b]{0.49\textwidth}
		\centering
		\includegraphics[width=\textwidth]{Figures/absolute_bias_tau.pdf}
		\caption{$\tau$}
		\label{fig:bias.tau}
	\end{subfigure}
	\caption{Absolute bias for the ATE point estimate produced by each estimator, divided by the different DGP parameters}
	\label{fig:sim.bias.ate}
\end{figure}

==> Figures/sim_rmse_cate.tex <==
\begin{figure}[!htpb]
	\centering
	\includegraphics[width=0.75\linewidth]{Figures/sim_intervals_cate.pdf}
	\caption{RMSE for the CATE point estimates produced by each estimator, divided by different levels of heterogenety (\textit{i.e.} $\kappa$)}
	\label{fig:sim.rmse.cate}
\end{figure}

==> Figures/sim_y.tex <==
\begin{figure}[!htpb]
	\centering
	\includegraphics[width=0.7\textwidth]{Figures/sim_y.pdf}
	\caption{$Y$ distribution}
	\label{fig:sim.y}
\end{figure}

==> Figures/trees.tex <==
\begin{figure}
	\centering
	\begin{subfigure}[b]{0.45\linewidth}
		\centering
		\includegraphics[width=\linewidth]{Figures/bad_trees_1a.pdf}
		\caption{}
		\label{fig:bad.1a}
	\end{subfigure}
	\hfill
	\begin{subfigure}[b]{0.45\linewidth}
		\centering
		\includegraphics[width=\linewidth]{Figures/bad_trees_1b.pdf}
		\caption{}
		\label{fig:bad.1b}
	\end{subfigure}
	\hfill
	\begin{subfigure}[b]{0.45\linewidth}
		\centering
		\includegraphics[width=\linewidth]{Figures/bad_trees_1c.pdf}
		\caption{}
		\label{fig:bad.1c}
	\end{subfigure}
	\hfill
	\begin{subfigure}[b]{0.45\linewidth}
		\centering
		\includegraphics[width=\linewidth]{Figures/good_tree_1.pdf}
		\caption{}
		\label{fig:good.1}
	\end{subfigure}
	\caption{Tree examples: the first and third trees show splits that violate condition ii, which can be accepted because we can make these trees valid by trimming out the region outside the identification strip in the relevant nodes; the second tree presents a set of splits that violates condition i, so it can never be made valid and is thus rejected; the fourth tree is an example of the kind of tree that would be accepted by the algorithm, with tight bounds on the identification region and good representation from both sides of the cutoff}
	\label{fig:tree.graphs}
\end{figure}

==> Tables/cor_sim.tex <==
\begin{table}[!htbp] \centering 
	\caption{Correlations between $Y$ and $(X,W)$} 
	\label{tab:cor.sim} 
	\begin{tabular}{@{\extracolsep{5pt}} c|c|ccccc} 
		$\kappa$ & $\nu$ & $X$ & $W_1$ & $W_2$ & $W_3$ & $W_4$
		\\
		\hline
		& 0.5 & 0.41 & -0.02 & 0.06 & 0.01 & 0.05 \\ 
		0 & 1 & 0.71 & -0.03 & -0.01 & -0.01 & -0.02 \\ 
		& 2 & 0.88 & 0.03 & 0.03 & -0.06 & -0.05 \\
		\hline
		& 0.5 & 0.38 & 0.14 & 0.05 & 0.14 & 0.01 \\ 
		1 & 1 & 0.61 & 0.19 & 0.24 & 0.25 & 0.09 \\ 
		& 2 & 0.72 & 0.32 & 0.3 & 0.3 & 0.13 \\
		\hline
		& 0.5 & 0.25 & 0.18 & 0.22 & 0.22 & 0.05 \\ 
		2 & 1 & 0.41 & 0.32 & 0.32 & 0.34 & 0.12 \\ 
		& 2 & 0.5 & 0.41 & 0.38 & 0.41 & 0.24 \\ 
		\hline
	\end{tabular} 
\end{table}

==> Tables/descriptive.tex <==
\begin{table}[ht]
	\centering
	\begin{tabular}{lcccccccc}
		\hline
		& \multicolumn{2}{c}{(1)} && \multicolumn{2}{c}{(2)} && \multicolumn{2}{c}{(3)}\\
		\cline{2-3} \cline{5-6} \cline{8-9} \\[-2.5ex]
		& Mean & Std. Dev & & Mean & Std. Dev & & Mean & Std. Dev \\ 
		\hline
		Next Term GPA & 2.57 & 0.91 &  & 1.95 & 0.81 &  & 1.98 & 0.8 \\ 
		Distance from cutoff & -0.96 & 0.86 &  & 0 & 0.05 &  & -0.08 & 0.26 \\ 
		Treatment assignment & 0.14 & 0.35 &  & 0.41 & 0.49 &  & 0.36 & 0.48 \\ 
		High school grade percentile & 51 & 28.71 &  & 31.65 & 22.79 &  & 32.76 & 23.15 \\ 
		Credits attempted in first year & 4.58 & 0.51 &  & 4.39 & 0.54 &  & 4.42 & 0.53 \\ 
		Age at entry & 18.66 & 0.74 &  & 18.72 & 0.75 &  & 18.71 & 0.74 \\ 
		Male & 0.38 & 0.49 &  & 0.38 & 0.48 &  & 0.37 & 0.48 \\ 
		Born in North America & 0.87 & 0.34 &  & 0.87 & 0.34 &  & 0.87 & 0.34 \\ 
		Campus 1 & 0.59 & 0.49 &  & 0.45 & 0.5 &  & 0.47 & 0.5 \\ 
		Campus 2 & 0.17 & 0.38 &  & 0.21 & 0.41 &  & 0.21 & 0.41 \\ 
		Campus 3 & 0.24 & 0.42 &  & 0.34 & 0.47 &  & 0.32 & 0.46 \\ 
		\hline
	\end{tabular}
	\caption{Descriptive statistics} 
	\label{tab:desc.stats}
\end{table}

==> Tables/gpa_results.tex <==
\begin{table}[ht]
	\centering
	\begin{tabular}{lccccc}
		\hline \\[-2.5ex]
		& Controls & $\hat{\tau}$ & 95\% CI & h & N \\ 
		\hline \\[-2.5ex]
		\multirow{2}*{BART-RDD} & No & 0.11 & [0.04,0.17] & 0.1 & 1757 \\ 
		& Yes & 0.13 & [0.08,0.2] & 0.1 & 1757 \\ 
		\multirow{2}*{CKT} & No & 0.22 & [0.13,0.3] & 0.47 & 8776 \\ 
		& Yes & 0.22 & [0.12,0.3] & 0.46 & 8776 \\ 
		\hline
	\end{tabular}
	\caption{RD Estimates} 
	\label{tab:gpa.res}
\end{table}

==> Tables/gpa_robust_1.tex <==
\begin{table}[ht]
	\centering
	\begin{tabular}{ccccc}
		\hline
		Controls & $N_{Omin}$ & $h$ & $\hat{\tau}$ & 95\% CI \\
		\hline
		\multirow{8}{*}{No} & \multirow{4}{*}{10} & 0.09 & 0.11 & [0.02,0.19] \\ 
		 & & 0.1 & 0.11 & [0.04,0.17] \\ 
		 & & 0.11 & 0.12 & [0.06,0.19] \\ 
		 & & 0.12 & 0.13 & [0.07,0.18] \\ 
		 \cline{2-5}
		 & \multirow{4}{*}{50} & 0.09 & 0.13 & [0.06,0.19] \\ 
		 & & 0.1 & 0.12 & [0.06,0.18] \\ 
		 & & 0.11 & 0.12 & [0.08,0.18] \\ 
		 & & 0.12 & 0.09 & [0.01,0.17] \\ 
		 \hline
		\multirow{8}{*}{Yes} & \multirow{4}{*}{10} & 0.09 & 0.13 & [0.05,0.23] \\ 
		 & & 0.1 & 0.14 & [0.08,0.2] \\ 
		 & & 0.11 & 0.14 & [0.07,0.21] \\ 
		 & & 0.12 & 0.15 & [0.1,0.2] \\ 
		 \cline{2-5}
		 & \multirow{4}{*}{50} & 0.09 & 0.13 & [0.06,0.21] \\ 
		 & & 0.1 & 0.09 & [0.01,0.2] \\ 
		 & & 0.11 & 0.13 & [0.07,0.18] \\ 
		 & & 0.12 & 0.14 & [0.09,0.2] \\ 
		\hline
	\end{tabular}
	\caption{RD Estimates - Sensitivity analysis} 
	\label{tab:gpa.robust}
\end{table}

==> Tables/prior_rmse.tex <==
\begin{table}[!htbp] \centering 
	\caption{Candidate $h$ values and RMSE for each (X,W) sample} 
	\label{tab:rmse.prior} 
	\begin{tabular}{cccccc} 
		\hline
		\multicolumn{2}{c}{DGP 1} & \multicolumn{2}{c}{DGP 2} & \multicolumn{2}{c}{DGP 3}  \\
		\hline 
		h & RMSE & h & RMSE & h & RMSE \\
		\hline
		0.04 & 0.173 & 0.1 & 0.159 & 0.04 & 0.168 \\ 
		0.09 & 0.087 & 0.24 & 0.129 & 0.09 & 0.092 \\ 
		0.18 & 0.052 & 0.48 & 0.131 & 0.18 & 0.045 \\ 
		0.36 & 0.101 & 0.95 & 0.276 & 0.36 & 0.091 \\ 
		\hline
	\end{tabular} 
\end{table}

==> Tables/sim_1_10.tex <==
\begin{table}[!htpb]
	\centering
	\begin{tabular}{llccccc}
		\hline
		&  & Controls & MSE & Variance & Coverage & Size \\ 
		\hline
		\multirow{6}{*}{XBCF} & \multirow{2}{*}{DGP 1} & No & 0.003 & 0.003 & 86 & 0.16 \\ 
		&  & Yes & 0.004 & 0.003 & 78.6 & 0.15 \\
		& \multirow{2}{*}{DGP 2} & No & 0.017 & 0.017 & 93.5 & 0.47 \\ 
		&  & Yes & 0.011 & 0.01 & 88.3 & 0.33 \\ 
		& \multirow{2}{*}{DGP 3} & No & 0.003 & 0.003 & 100 & 0.63 \\ 
		&  & Yes & 0.015 & 0.003 & 100 & 0.7 \\ 
		\hline
		\multirow{6}{*}{BART} & \multirow{2}{*}{DGP 1} & No & 0.002 & 0.002 & 97.7 & 0.26 \\ 
		&  & Yes & 0.002 & 0.002 & 96 & 0.19 \\ 
		& \multirow{2}{*}{DGP 2} & No & 0.295 & 0.056 & 66 & 1.06 \\ 
		&  & Yes & 0.296 & 0.029 & 86.8 & 1.12 \\ 
		& \multirow{2}{*}{DGP 3} & No & 0.935 & 0.051 & 99.4 & 2.47 \\ 
		&  & Yes & 0.886 & 0.053 & 99.2 & 2.39 \\ 
		\hline
		\multirow{6}{*}{BART2} & \multirow{2}{*}{DGP 1} & No & 0.008 & 0.004 & 86.4 & 0.28 \\ 
		&  & Yes & 0.019 & 0.002 & 39.5 & 0.22 \\ 
		& \multirow{2}{*}{DGP 2} & No & 0.019 & 0.019 & 91.9 & 0.5 \\ 
		&  & Yes & 0.012 & 0.004 & 71.3 & 0.27 \\ 
		& \multirow{2}{*}{DGP 3} & No & 0.007 & 0.003 & 96 & 0.39 \\ 
		&  & Yes & 0.023 & 0.001 & 32.8 & 0.24 \\
		\hline
		\multirow{6}{*}{BCF} & \multirow{2}{*}{DGP 1} & No & 0.01 & 0.006 & 66.9 & 0.16 \\ 
		&  & Yes & 0.018 & 0.008 & 45.1 & 0.15 \\ 
		& \multirow{2}{*}{DGP 2} & No & 0.302 & 0.186 & 55.5 & 0.72 \\ 
		&  & Yes & 0.553 & 0.159 & 19 & 0.39 \\ 
		& \multirow{2}{*}{DGP 3} & No & 2.886 & 0.884 & 24.9 & 0.85 \\ 
		&  & Yes & 2.892 & 0.978 & 26.7 & 0.83 \\ 
		\hline
		\multirow{6}{*}{CGS} & \multirow{2}{*}{DGP 1} & No & 0.03 & 0.03 & 95.9 & 0.65 \\ 
		&  & Yes & 0.03 & 0.03 & 96.9 & 0.63 \\ 
		& \multirow{2}{*}{DGP 2} & No & 0.09 & 0.09 & 96.9 & 1.32 \\ 
		&  & Yes & 0.04 & 0.04 & 96.2 & 0.81 \\ 
		& \multirow{2}{*}{DGP 3} & No & 0.03 & 0.03 & 98.1 & 0.79 \\ 
		&  & Yes & 0.01 & 0.01 & 99.8 & 0.59 \\ 
		\hline
		\multirow{6}{*}{KR} & \multirow{2}{*}{DGP 1} & No & 0.026 & 0.026 & 93.3 & 0.49 \\ 
		&  & Yes & 0.026 & 0.026 & 93 & 0.49 \\ 
		& \multirow{2}{*}{DGP 2} & No & 0.115 & 0.115 & 92.5 & 1.27 \\ 
		&  & Yes & 0.038 & 0.037 & 89.8 & 0.66 \\ 
		& \multirow{2}{*}{DGP 3} & No & 0.016 & 0.016 & 92.2 & 0.48 \\ 
		&  & Yes & 0.006 & 0.006 & 83.9 & 0.21 \\ 
		\hline
		\multirow{6}{*}{CKT} & \multirow{2}{*}{DGP 1} & No & 0.011 & 0.011 & 93.1 & 0.4 \\ 
		&  & Yes & 0.014 & 0.013 & 87.3 & 0.37 \\ 
		& \multirow{2}{*}{DGP 2} & No & 0.058 & 0.057 & 91.9 & 0.95 \\ 
		&  & Yes & 0.021 & 0.021 & 86.9 & 0.51 \\ 
		& \multirow{2}{*}{DGP 3} & No & 0.008 & 0.008 & 91.3 & 0.38 \\ 
		&  & Yes & 0.003 & 0.002 & 85.2 & 0.17 \\ 
		\hline
	\end{tabular}
	\caption{Simulation results for P=10} 
	\label{tab:sim.1.10}
\end{table}

==> Tables/sim_1_4.tex <==
\begin{table}[!htpb]
	\centering
	\begin{tabular}{llccccc}
		\hline
		&  & Controls & MSE & Variance & Coverage & Size \\ 
		\hline
		\multirow{6}{*}{XBCF} & \multirow{2}{*}{DGP 1} & No & 0.003 & 0.003 & 87.4 & 0.16 \\ 
		&  & Yes & 0.004 & 0.003 & 82.5 & 0.15 \\ 
		& \multirow{2}{*}{DGP 2} & No & 0.017 & 0.017 & 92.9 & 0.47 \\ 
		&  & Yes & 0.011 & 0.01 & 89.4 & 0.33 \\ 
		& \multirow{2}{*}{DGP 3} & No & 0.003 & 0.003 & 100 & 0.64 \\ 
		&  & Yes & 0.008 & 0.003 & 100 & 0.68 \\ 
		\hline
		\multirow{6}{*}{BART} & \multirow{2}{*}{DGP 1} & No & 0.002 & 0.002 & 97.8 & 0.26 \\ 
		&  & Yes & 0.002 & 0.002 & 97.9 & 0.2 \\ 
		& \multirow{2}{*}{DGP 2} & No & 0.297 & 0.051 & 65.9 & 1.07 \\ 
		&  & Yes & 0.29 & 0.029 & 85.2 & 1.11 \\ 
		& \multirow{2}{*}{DGP 3} & No & 0.884 & 0.054 & 99.1 & 2.46 \\ 
		&  & Yes & 0.882 & 0.052 & 99.3 & 2.36 \\ 
		\hline
		\multirow{6}{*}{BART2} & \multirow{2}{*}{DGP 1} & No & 0.008 & 0.004 & 88.5 & 0.28 \\ 
		&  & Yes & 0.014 & 0.002 & 58.8 & 0.24 \\ 
		& \multirow{2}{*}{DGP 2} & No & 0.018 & 0.018 & 93.1 & 0.5 \\ 
		&  & Yes & 0.01 & 0.005 & 82.4 & 0.29 \\ 
		& \multirow{2}{*}{DGP 3} & No & 0.007 & 0.003 & 96.3 & 0.39 \\ 
		&  & Yes & 0.02 & 0.001 & 48.9 & 0.25 \\ 
		\hline
		\multirow{6}{*}{BCF} & \multirow{2}{*}{DGP 1} & No & 0.01 & 0.006 & 67.2 & 0.16 \\ 
		&  & Yes & 0.014 & 0.007 & 55.4 & 0.16 \\ 
		& \multirow{2}{*}{DGP 2} & No & 0.303 & 0.19 & 54.8 & 0.7 \\ 
		&  & Yes & 0.528 & 0.155 & 16.5 & 0.39 \\ 
		& \multirow{2}{*}{DGP 3} & No & 2.847 & 0.994 & 27.9 & 0.85 \\ 
		&  & Yes & 2.904 & 0.996 & 27.6 & 0.83 \\
		\hline
		\multirow{6}{*}{CGS} & \multirow{2}{*}{DGP 1} & No & 0.02 & 0.02 & 96.3 & 0.65 \\ 
		&  & Yes & 0.02 & 0.02 & 96.7 & 0.65 \\ 
		& \multirow{2}{*}{DGP 2} & No & 0.09 & 0.09 & 97.3 & 1.34 \\ 
		&  & Yes & 0.04 & 0.04 & 96 & 0.82 \\ 
		& \multirow{2}{*}{DGP 3} & No & 0.04 & 0.03 & 97.2 & 0.81 \\ 
		&  & Yes & 0.01 & 0.01 & 99.5 & 0.6 \\
		\hline
		\multirow{6}{*}{KR} & \multirow{2}{*}{DGP 1} & No & 0.019 & 0.019 & 93.8 & 0.49 \\ 
		&  & Yes & 0.019 & 0.019 & 93.7 & 0.49 \\ 
		& \multirow{2}{*}{DGP 2} & No & 0.116 & 0.116 & 92.9 & 1.21 \\ 
		&  & Yes & 0.042 & 0.042 & 91.5 & 0.68 \\ 
		& \multirow{2}{*}{DGP 3} & No & 0.017 & 0.017 & 92.9 & 0.49 \\ 
		&  & Yes & 0.006 & 0.006 & 87 & 2.97 \\
		\hline
		\multirow{6}{*}{CKT} & \multirow{2}{*}{DGP 1} & No & 0.01 & 0.009 & 93.8 & 0.4 \\ 
		&  & Yes & 0.01 & 0.01 & 91.8 & 0.39 \\ 
		& \multirow{2}{*}{DGP 2} & No & 0.057 & 0.057 & 91.9 & 0.96 \\ 
		&  & Yes & 0.019 & 0.019 & 90.6 & 0.53 \\ 
		& \multirow{2}{*}{DGP 3} & No & 0.008 & 0.008 & 92.3 & 0.39 \\ 
		&  & Yes & 0.002 & 0.002 & 90.8 & 0.2 \\ 
		\hline
	\end{tabular}
	\caption{Simulation results for P=4} 
	\label{tab:sim.1.4}
\end{table}

==> Tables/sim_1_6.tex <==
\begin{table}[!htpb]
	\centering
	\begin{tabular}{llccccc}
		\hline
		&  & Controls & MSE & Variance & Coverage & Size \\ 
		\hline
		\multirow{6}{*}{XBCF} & \multirow{2}{*}{DGP 1} & No & 0.004 & 0.003 & 87.7 & 0.16 \\ 
		&  & Yes & 0.004 & 0.003 & 79.9 & 0.15 \\ 
		& \multirow{2}{*}{DGP 2} & No & 0.017 & 0.017 & 92.4 & 0.47 \\ 
		&  & Yes & 0.011 & 0.01 & 89.5 & 0.33 \\ 
		& \multirow{2}{*}{DGP 3} & No & 0.003 & 0.003 & 100 & 0.63 \\ 
		&  & Yes & 0.011 & 0.003 & 100 & 0.69 \\ 
		\hline
		\multirow{6}{*}{BART} & \multirow{2}{*}{DGP 1} & No & 0.006 & 0.006 & 97.3 & 0.26 \\ 
		&  & Yes & 0.002 & 0.002 & 97.2 & 0.2 \\ 
		& \multirow{2}{*}{DGP 2} & No & 0.293 & 0.055 & 65.4 & 1.07 \\ 
		&  & Yes & 0.278 & 0.026 & 86.9 & 1.12 \\ 
		& \multirow{2}{*}{DGP 3} & No & 0.92 & 0.053 & 98.9 & 2.43 \\ 
		&  & Yes & 0.879 & 0.051 & 99.5 & 2.39 \\
		\hline
		\multirow{6}{*}{BART2} & \multirow{2}{*}{DGP 1} & No & 0.008 & 0.004 & 85.3 & 0.28 \\ 
		&  & Yes & 0.016 & 0.002 & 50.1 & 0.23 \\ 
		& \multirow{2}{*}{DGP 2} & No & 0.019 & 0.018 & 91.4 & 0.5 \\ 
		&  & Yes & 0.011 & 0.004 & 76.7 & 0.28 \\ 
		& \multirow{2}{*}{DGP 3} & No & 0.006 & 0.003 & 97.8 & 0.39 \\ 
		&  & Yes & 0.021 & 0.001 & 37.9 & 0.24 \\
		\hline
		\multirow{6}{*}{BCF} & \multirow{2}{*}{DGP 1} & No & 0.042 & 0.038 & 66 & 0.16 \\ 
		&  & Yes & 0.015 & 0.008 & 52.4 & 0.15 \\ 
		& \multirow{2}{*}{DGP 2} & No & 0.308 & 0.193 & 54.6 & 0.7 \\ 
		&  & Yes & 0.544 & 0.158 & 16.2 & 0.37 \\ 
		& \multirow{2}{*}{DGP 3} & No & 2.825 & 0.913 & 26.9 & 0.85 \\ 
		&  & Yes & 2.781 & 0.971 & 29 & 0.83 \\ 
		\hline
		\multirow{6}{*}{CGS} & \multirow{2}{*}{DGP 1} & No & 0.02 & 0.02 & 96.3 & 0.66 \\ 
		&  & Yes & 0.02 & 0.02 & 97.5 & 0.64 \\ 
		& \multirow{2}{*}{DGP 2} & No & 0.08 & 0.08 & 97.6 & 1.31 \\ 
		&  & Yes & 0.04 & 0.04 & 95.9 & 0.8 \\ 
		& \multirow{2}{*}{DGP 3} & No & 0.03 & 0.03 & 97 & 0.81 \\ 
		&  & Yes & 0.01 & 0.01 & 99.4 & 0.6 \\
		\hline
		\multirow{6}{*}{KR} & \multirow{2}{*}{DGP 1} & No & 0.022 & 0.022 & 93.5 & 0.5 \\ 
		&  & Yes & 0.022 & 0.022 & 93.3 & 0.49 \\ 
		& \multirow{2}{*}{DGP 2} & No & 0.101 & 0.101 & 93.3 & 1.17 \\ 
		&  & Yes & 0.041 & 0.041 & 89.7 & 0.66 \\ 
		& \multirow{2}{*}{DGP 3} & No & 0.018 & 0.018 & 93.3 & 0.5 \\ 
		&  & Yes & 0.006 & 0.006 & 86.7 & 0.53 \\ 
		\hline
		\multirow{6}{*}{CKT} & \multirow{2}{*}{DGP 1} & No & 0.01 & 0.01 & 93.7 & 0.4 \\ 
		&  & Yes & 0.012 & 0.011 & 89.7 & 0.38 \\ 
		& \multirow{2}{*}{DGP 2} & No & 0.051 & 0.051 & 93.2 & 0.94 \\ 
		&  & Yes & 0.019 & 0.019 & 88.8 & 0.52 \\ 
		& \multirow{2}{*}{DGP 3} & No & 0.009 & 0.009 & 91.8 & 0.39 \\ 
		&  & Yes & 0.003 & 0.003 & 87.4 & 0.19 \\ 
		\hline
	\end{tabular}
	\caption{Simulation results for P=6} 
	\label{tab:sim.1.6}
\end{table}

==> Tables/sim_2_10.tex <==
\begin{table}[!htpb]
	\centering
	\begin{tabular}{llccccc}
		\hline
		&  & Controls & MSE & Variance & Coverage & Size \\ 
		\hline
		\multirow{6}{*}{XBCF} & \multirow{2}{*}{DGP 4} & No & 0.082 & 0.083 & 93.1 & 1.04 \\ 
		&  & Yes & 0.069 & 0.07 & 92.9 & 0.95 \\ 
		& \multirow{2}{*}{DGP 5} & No & 0.077 & 0.079 & 93.4 & 1.04 \\ 
		&  & Yes & 0.071 & 0.07 & 93 & 0.96 \\ 
		& \multirow{2}{*}{DGP 6} & No & 0.086 & 0.087 & 93.8 & 1.11 \\ 
		&  & Yes & 0.073 & 0.074 & 93.6 & 1 \\ 
		\hline
		\multirow{6}{*}{BART} & \multirow{2}{*}{DGP 4} & No & 0.291 & 0.085 & 81.3 & 1.4 \\ 
		&  & Yes & 0.411 & 0.08 & 74 & 1.27 \\ 
		& \multirow{2}{*}{DGP 5} & No & 0.432 & 0.104 & 73.5 & 1.52 \\ 
		&  & Yes & 0.521 & 0.09 & 69.2 & 1.33 \\ 
		& \multirow{2}{*}{DGP 6} & No & 0.584 & 0.129 & 73.4 & 1.72 \\ 
		&  & Yes & 0.743 & 0.115 & 64.9 & 1.49 \\ 
		\hline
		\multirow{6}{*}{BART2} & \multirow{2}{*}{DGP 4} & No & 0.11 & 0.099 & 88.9 & 1.13 \\ 
		&  & Yes & 0.186 & 0.051 & 54.1 & 0.8 \\ 
		& \multirow{2}{*}{DGP 5} & No & 0.099 & 0.097 & 91.1 & 1.14 \\ 
		&  & Yes & 0.168 & 0.064 & 67.6 & 0.92 \\ 
		& \multirow{2}{*}{DGP 6} & No & 0.109 & 0.102 & 90.8 & 1.2 \\ 
		&  & Yes & 0.17 & 0.065 & 67.5 & 0.92 \\
		\hline
		\multirow{6}{*}{BCF} & \multirow{2}{*}{DGP 4} & No & 0.242 & 0.084 & 42.4 & 0.81 \\ 
		&  & Yes & 0.317 & 0.075 & 25.3 & 0.7 \\ 
		& \multirow{2}{*}{DGP 5} & No & 0.3 & 0.173 & 49.6 & 0.96 \\ 
		&  & Yes & 0.367 & 0.132 & 32 & 0.82 \\ 
		& \multirow{2}{*}{DGP 6} & No & 0.296 & 0.145 & 47.5 & 0.97 \\ 
		&  & Yes & 0.344 & 0.157 & 33.1 & 0.87 \\ 
		\hline
		\multirow{6}{*}{CGS} & \multirow{2}{*}{DGP 4} & No & 0.44 & 0.43 & 94.8 & 2.6 \\ 
		&  & Yes & 0.4 & 0.4 & 95.7 & 2.55 \\ 
		& \multirow{2}{*}{DGP 5} & No & 0.48 & 0.48 & 93.9 & 2.72 \\ 
		&  & Yes & 0.42 & 0.43 & 95 & 2.63 \\ 
		& \multirow{2}{*}{DGP 6} & No & 0.58 & 0.58 & 93.3 & 2.78 \\ 
		&  & Yes & 0.49 & 0.49 & 94.1 & 2.68 \\ 
		\hline
		\multirow{6}{*}{KR} & \multirow{2}{*}{DGP 4} & No & 0.586 & 0.589 & 94.1 & 2.79 \\ 
		&  & Yes & 0.599 & 0.601 & 93.2 & 2.75 \\ 
		& \multirow{2}{*}{DGP 5} & No & 0.575 & 0.571 & 92.3 & 2.77 \\ 
		&  & Yes & 0.572 & 0.569 & 91.4 & 2.71 \\ 
		& \multirow{2}{*}{DGP 6} & No & 0.68 & 0.684 & 94.2 & 2.97 \\ 
		&  & Yes & 0.688 & 0.691 & 92.9 & 2.89 \\ 
		\hline
		\multirow{6}{*}{CKT} & \multirow{2}{*}{DGP 4} & No & 0.29 & 0.293 & 93.1 & 2.24 \\ 
		&  & Yes & 0.315 & 0.318 & 87.7 & 1.94 \\ 
		& \multirow{2}{*}{DGP 5} & No & 0.276 & 0.274 & 91.9 & 2.21 \\ 
		&  & Yes & 0.303 & 0.3 & 87.1 & 1.94 \\ 
		& \multirow{2}{*}{DGP 6} & No & 0.317 & 0.318 & 93.4 & 2.36 \\ 
		&  & Yes & 0.305 & 0.305 & 88.4 & 2.01 \\ 
		\hline
	\end{tabular}
	\caption{Simulation results for P=10} 
	\label{tab:sim.2.10}
\end{table}

==> Tables/sim_2_4.tex <==
\begin{table}[!htpb]
	\centering
	\begin{tabular}{llccccc}
		\hline
		&  & Controls & MSE & Variance & Coverage & Size \\ 
		\hline
		\multirow{6}{*}{XBCF} & \multirow{2}{*}{DGP 4} & No & 0.089 & 0.09 & 92.1 & 1.07 \\ 
		&  & Yes & 0.068 & 0.069 & 91.8 & 0.92 \\ 
		& \multirow{2}{*}{DGP 5} & No & 0.089 & 0.084 & 91.4 & 1.07 \\ 
		&  & Yes & 0.089 & 0.071 & 87.8 & 0.96 \\ 
		& \multirow{2}{*}{DGP 6} & No & 0.103 & 0.1 & 92.7 & 1.17 \\ 
		&  & Yes & 0.086 & 0.077 & 88.9 & 0.99 \\ 
		\hline
		\multirow{6}{*}{BART} & \multirow{2}{*}{DGP 4} & No & 0.299 & 0.092 & 79.8 & 1.42 \\ 
		&  & Yes & 0.379 & 0.087 & 74.8 & 1.34 \\ 
		& \multirow{2}{*}{DGP 5} & No & 0.526 & 0.108 & 67.5 & 1.57 \\ 
		&  & Yes & 0.598 & 0.094 & 65.6 & 1.42 \\ 
		& \multirow{2}{*}{DGP 6} & No & 0.716 & 0.138 & 65.8 & 1.74 \\ 
		&  & Yes & 0.856 & 0.116 & 58.6 & 1.57 \\ 
		\hline
		\multirow{6}{*}{BART2} & \multirow{2}{*}{DGP 4} & No & 0.122 & 0.109 & 88.3 & 1.15 \\ 
		&  & Yes & 0.138 & 0.054 & 65 & 0.82 \\ 
		& \multirow{2}{*}{DGP 5} & No & 0.109 & 0.11 & 89.9 & 1.16 \\ 
		&  & Yes & 0.116 & 0.077 & 82.6 & 0.98 \\ 
		& \multirow{2}{*}{DGP 6} & No & 0.119 & 0.12 & 90.7 & 1.26 \\ 
		&  & Yes & 0.112 & 0.07 & 84.2 & 0.98 \\ 
		\hline
		\multirow{6}{*}{BCF} & \multirow{2}{*}{DGP 4} & No & 0.248 & 0.087 & 44.5 & 0.84 \\ 
		&  & Yes & 0.282 & 0.096 & 35.1 & 0.78 \\ 
		& \multirow{2}{*}{DGP 5} & No & 0.265 & 0.187 & 55.1 & 1.03 \\ 
		&  & Yes & 0.218 & 0.156 & 58.6 & 0.97 \\ 
		& \multirow{2}{*}{DGP 6} & No & 0.264 & 0.159 & 54 & 1.02 \\ 
		&  & Yes & 0.247 & 0.224 & 58.6 & 1 \\ 
		\hline
		\multirow{6}{*}{CGS} & \multirow{2}{*}{DGP 4} & No & 0.53 & 0.53 & 93 & 2.64 \\ 
		&  & Yes & 0.41 & 0.41 & 94.7 & 2.52 \\ 
		& \multirow{2}{*}{DGP 5} & No & 0.61 & 0.6 & 93 & 2.85 \\ 
		&  & Yes & 0.46 & 0.45 & 95.3 & 2.61 \\ 
		& \multirow{2}{*}{DGP 6} & No & 0.68 & 0.67 & 92.3 & 2.92 \\ 
		&  & Yes & 0.49 & 0.49 & 94.1 & 2.68 \\ 
		\hline
		\multirow{6}{*}{KR} & \multirow{2}{*}{DGP 4} & No & 0.671 & 0.671 & 91.8 & 2.86 \\ 
		&  & Yes & 0.601 & 0.602 & 91.3 & 2.63 \\ 
		& \multirow{2}{*}{DGP 5} & No & 0.718 & 0.694 & 92.7 & 186.03 \\ 
		&  & Yes & 0.681 & 0.657 & 90.2 & 2.67 \\ 
		& \multirow{2}{*}{DGP 6} & No & 0.791 & 0.784 & 92.6 & 3.07 \\ 
		&  & Yes & 0.758 & 0.752 & 91 & 28.48 \\ 
		\hline
		\multirow{6}{*}{CKT} & \multirow{2}{*}{DGP 4} & No & 0.33 & 0.33 & 91.6 & 2.29 \\ 
		&  & Yes & 0.247 & 0.247 & 91.8 & 1.95 \\ 
		& \multirow{2}{*}{DGP 5} & No & 0.35 & 0.327 & 91.5 & 2.31 \\ 
		&  & Yes & 0.289 & 0.263 & 90.1 & 1.97 \\ 
		& \multirow{2}{*}{DGP 6} & No & 0.388 & 0.383 & 91.8 & 2.47 \\ 
		&  & Yes & 0.288 & 0.283 & 90.5 & 2.06 \\ 
		\hline
	\end{tabular}
	\caption{Simulations results for P=4} 
	\label{tab:sim.2.4}
\end{table}

==> Tables/sim_2_6.tex <==
\begin{table}[!htpb]
	\centering
	\begin{tabular}{llccccc}
		\hline
		&  & Controls & MSE & Variance & Coverage & Size \\ 
		\hline
		\multirow{6}{*}{XBCF} & \multirow{2}{*}{DGP 4} & No & 0.081 & 0.082 & 92.4 & 1.06 \\ 
		&  & Yes & 0.063 & 0.064 & 92.9 & 0.93 \\ 
		& \multirow{2}{*}{DGP 5} & No & 0.088 & 0.086 & 92.2 & 1.06 \\ 
		&  & Yes & 0.082 & 0.072 & 90 & 0.96 \\ 
		& \multirow{2}{*}{DGP 6} & No & 0.098 & 0.098 & 92.2 & 1.15 \\ 
		&  & Yes & 0.086 & 0.08 & 89.8 & 0.98 \\ 
		\hline
		\multirow{6}{*}{BART} & \multirow{2}{*}{DGP 4} & No & 0.302 & 0.095 & 79 & 1.4 \\ 
		&  & Yes & 0.397 & 0.087 & 74.1 & 1.29 \\ 
		& \multirow{2}{*}{DGP 5} & No & 0.475 & 0.106 & 71.1 & 1.56 \\ 
		&  & Yes & 0.576 & 0.092 & 63.3 & 1.38 \\ 
		& \multirow{2}{*}{DGP 6} & No & 0.64 & 0.131 & 71 & 1.73 \\ 
		&  & Yes & 0.778 & 0.114 & 63.1 & 1.54 \\ 
		\hline
		\multirow{6}{*}{BART2} & \multirow{2}{*}{DGP 4} & No & 0.108 & 0.099 & 90.2 & 1.13 \\ 
		&  & Yes & 0.159 & 0.051 & 60.1 & 0.81 \\ 
		& \multirow{2}{*}{DGP 5} & No & 0.107 & 0.108 & 90.2 & 1.15 \\ 
		&  & Yes & 0.135 & 0.076 & 77.2 & 0.95 \\ 
		& \multirow{2}{*}{DGP 6} & No & 0.115 & 0.116 & 91 & 1.24 \\ 
		&  & Yes & 0.134 & 0.072 & 77.8 & 0.95 \\ 
		\hline
		\multirow{6}{*}{BCF} & \multirow{2}{*}{DGP 4} & No & 0.246 & 0.083 & 44.6 & 0.83 \\ 
		&  & Yes & 0.299 & 0.093 & 32 & 0.75 \\ 
		& \multirow{2}{*}{DGP 5} & No & 0.278 & 0.172 & 54.4 & 1 \\ 
		&  & Yes & 0.293 & 0.154 & 44.1 & 0.93 \\ 
		& \multirow{2}{*}{DGP 6} & No & 0.285 & 0.166 & 49.2 & 1 \\ 
		&  & Yes & 0.287 & 0.194 & 43 & 0.92 \\ 
		\hline
		\multirow{6}{*}{CGS} & \multirow{2}{*}{DGP 4} & No & 0.45 & 0.45 & 95.4 & 2.67 \\ 
		&  & Yes & 0.37 & 0.38 & 95.5 & 2.58 \\ 
		& \multirow{2}{*}{DGP 5} & No & 0.56 & 0.55 & 93.8 & 2.74 \\ 
		&  & Yes & 0.45 & 0.44 & 94.3 & 2.6 \\ 
		& \multirow{2}{*}{DGP 6} & No & 0.64 & 0.63 & 92.1 & 2.85 \\ 
		&  & Yes & 0.5 & 0.5 & 93.8 & 2.67 \\ 
		\hline
		\multirow{6}{*}{KR} & \multirow{2}{*}{DGP 4} & No & 0.567 & 0.569 & 93.7 & 2.84 \\ 
		&  & Yes & 0.561 & 0.564 & 93.9 & 16.74 \\ 
		& \multirow{2}{*}{DGP 5} & No & 0.639 & 0.627 & 91.8 & 2.79 \\ 
		&  & Yes & 0.641 & 0.631 & 89.6 & 2.79 \\ 
		& \multirow{2}{*}{DGP 6} & No & 0.73 & 0.722 & 92.8 & 3.05 \\ 
		&  & Yes & 0.686 & 0.677 & 91.4 & 2.81 \\ 
		\hline
		\multirow{6}{*}{CKT} & \multirow{2}{*}{DGP 4} & No & 0.281 & 0.283 & 93.7 & 2.28 \\ 
		&  & Yes & 0.237 & 0.238 & 91.3 & 1.97 \\ 
		& \multirow{2}{*}{DGP 5} & No & 0.319 & 0.303 & 91.4 & 2.25 \\ 
		&  & Yes & 0.282 & 0.268 & 90 & 1.95 \\ 
		& \multirow{2}{*}{DGP 6} & No & 0.349 & 0.342 & 93 & 2.43 \\ 
		&  & Yes & 0.293 & 0.287 & 90.1 & 2.02 \\ 
		\hline
	\end{tabular}
	\caption{Simulation results for P=6} 
	\label{tab:sim.2.6}
\end{table}

==> Tables/sim_coverage_ate.tex <==
% Table created by stargazer v.5.2.3 by Marek Hlavac, Social Policy Institute. E-mail: marek.hlavac at gmail.com
% Date and time: qui, jun 13, 2024 - 22:37:02
\begin{table}[!htbp] \centering 
	\caption{Coverage rate for the ATE} 
	\label{tab:sim.coverage} 
	\small
	\begin{tabular}{@{\extracolsep{5pt}} ccccccccc} 
		\hline
		$\bar{\tau}$ & $\delta_{\mu}$ & $\delta_{\tau}$ & BART-RDD & S-BART & T-BART & CGS & LLR \\ 
		\hline \\[-1.8ex] 
		$0.2$ & $0.5$ & $0.1$ & $0.924$ & $0.954$ & $0.798$ & $0.962$ & $0.940$ \\ 
		$0.2$ & $0.5$ & $0.3$ & $0.954$ & $0.950$ & $0.724$ & $0.950$ & $0.932$ \\ 
		$0.2$ & $1.25$ & $0.1$ & $0.782$ & $0.940$ & $0.538$ & $0.970$ & $0.930$ \\ 
		$0.2$ & $1.25$ & $0.3$ & $0.718$ & $0.950$ & $0.520$ & $0.964$ & $0.938$ \\ 
		$0.5$ & $0.5$ & $0.1$ & $0.900$ & $0.866$ & $0.828$ & $0.958$ & $0.946$ \\ 
		$0.5$ & $0.5$ & $0.3$ & $0.920$ & $0.890$ & $0.772$ & $0.962$ & $0.942$ \\ 
		$0.5$ & $1.25$ & $0.1$ & $0.722$ & $0.870$ & $0.558$ & $0.966$ & $0.918$ \\ 
		$0.5$ & $1.25$ & $0.3$ & $0.702$ & $0.894$ & $0.572$ & $0.962$ & $0.934$ \\ 
		\hline
	\end{tabular} 
\end{table} 

==> Tables/sim_het.tex <==
\begin{table}[ht]
	\centering
	\begin{tabular}{lcccccccc}
		\hline \\[-2.5ex]
		&  & \multicolumn{3}{c}{ATE} &  & \multicolumn{3}{c}{CATE}\\
		\cline{3-5} \cline{7-9} \\[-2.5ex]
		&  & MSE & Coverage & Size &  & MSE & Coverage & Size \\
		\hline \\[-2.5ex]
		XBCF &  & 0.07 & 0.918 & 0.9 &  & 0.16 & 0.92 & 1.51 \\ 
		BART &  & 0.38 & 0.738 & 1.36 &  & 0.46 & 0.75 & 1.53 \\ 
		BCF &  & 0.16 & 0.528 & 0.78 &  & 0.28 & 0.55 & 0.86 \\ 
		\hline
	\end{tabular}
	\caption{Simulation results for CATE estimates} 
	\label{tab:sim.cate}
\end{table}

==> Tables/sim_int.tex <==
% Table created by stargazer v.5.2.3 by Marek Hlavac, Social Policy Institute. E-mail: marek.hlavac at gmail.com
% Date and time: sex, jun 14, 2024 - 11:08:37
\begin{table}[!htbp] \centering 
	\caption{Interval sizes for the ATE} 
	\label{tab:sim.int} 
	\small
	\begin{tabular}{@{\extracolsep{5pt}} cccccccc} 
		\hline
		$\tau$ & $\delta_{\mu}$ & $\delta_{\tau}$ & BART-RDD & S-BART & T-BART & CGS & LLR \\ 
		\hline \\[-1.8ex] 
		$0.2$ & $0.5$ & $0.1$ & $0.424$ & $0.713$ & $0.719$ & $1.598$ & $0.855$ \\ 
		$0.2$ & $0.5$ & $0.3$ & $0.442$ & $0.757$ & $0.677$ & $1.604$ & $0.877$ \\ 
		$0.2$ & $1.25$ & $0.1$ & $0.546$ & $0.970$ & $0.797$ & $1.792$ & $0.863$ \\ 
		$0.2$ & $1.25$ & $0.3$ & $0.539$ & $1.068$ & $0.794$ & $1.814$ & $0.880$ \\ 
		$0.5$ & $0.5$ & $0.1$ & $0.536$ & $0.859$ & $0.743$ & $1.604$ & $0.870$ \\ 
		$0.5$ & $0.5$ & $0.3$ & $0.519$ & $0.913$ & $0.704$ & $1.607$ & $0.870$ \\ 
		$0.5$ & $1.25$ & $0.1$ & $0.579$ & $1.239$ & $0.810$ & $1.788$ & $0.870$ \\ 
		$0.5$ & $1.25$ & $0.3$ & $0.567$ & $1.313$ & $0.818$ & $1.798$ & $0.872$ \\
		\hline \\[-1.8ex] 
	\end{tabular} 
\end{table} 
